Optimal stationary markings

Many specific problems ranging from theoretical probability to applications in statistical physics, combinatorial optimization and communications can be formulated as an optimal tuning of local parameters in large systems of interacting particles. Using the framework of stationary point processes in the Euclidean space, we pose it as a problem of an optimal stationary marking of a given stationary point process. The quality of a given marking is evaluated in terms of scores calculated in a covariant manner for all points in function of the proposed marked configuration. In the absence of total order of the configurations of scores, we identify intensity-optimality and local optimality as two natural ways for defining optimal stationary marking. We derive tightness and integrability conditions under which intensity-optimal markings exist and further stabilization conditions making them equivalent to locally optimal ones. We present examples motivating the proposed, general framework. Finally, we discuss various possible approaches leading to uniqueness results.

==> uniqueness.tex <==

\section{Uniqueness results}
\label{uniqSec}
\subsection{Proofs of Propositions \ref{prop.opt-MTP}--\ref{prop.uniq-MTP}}
In this section, we prove Propositions \ref{prop.opt-MTP}--\ref{prop.uniq-MTP} on optimal markings for score functions of mass-transport type.


\begin{proof}[Proof of Proposition \ref{prop.ex-MTP}]
First, assume that the considered $\arg\max$ is not empty.
Let $\mc M':\,\NM^0\longrightarrow[0, \infty)$ be defined such that $\mc  M'(\varphi)$ is the smallest element in $\arg\max_{m' \ge 0}f(m',\varphi)$. Then, the marking $\Psi$ with $M'_i:= \mc M'(\theta_{X_i}\Phi)$
is intensity-optimal. 
	
	On the other hand, consider
an intensity-optimal marking $\Psi$ and let $M'_0$ be
the value of the mark at the typical point under~$\P^0$. Then, by Proposition~\ref{prop.opt-MTP},
$$\E^0[f(M'_0,\Phi)] =
\sup_{\mc L(\Psi) \in \T(\Phi)}\frac1\la \gh(\Psi) =
\E^0[\sup_{m' \ge 0} f(m',\Phi)]\,,$$
and thus 
$f(M'_0,\Phi) = \sup_{m' \ge 0} f(m',\Phi)$ 
holds $\P^0_\Phi$ almost surely.
In particular,
$\arg\max_{m' \ge 0}\allowbreak f(m',\Phi) \ne \es$.
\end{proof}


\begin{proof}[Proof of Proposition \ref{prop.uniq-MTP}]
	Define the function $\mc M':\,\NM^0\longrightarrow[0, \infty)$ and the marking $\Psi = \{(X_i, M_i, M_i')\}_{i}$ as in the proof of Proposition \ref{prop.ex-MTP}.
	
	First, assume that $\arg\max_{m' \ge 0}f(m', \Phi)$ is $\P^0_\Phi$-almost surely unique. By Proposition~\ref{prop.opt-MTP} $M'_i$ is an intensity-optimal marking, and consider another intensity-optimal marking $\tilde\Psi = \{(X_i, M_i, \tilde M_i')\}_{i}$. Then,
	$$0 = \E^0[f(M'_0, \Phi) - f(\tilde M'_0, \Phi)],$$
	so that $\P^0$ almost surely $M'_0 = \tilde M'_0$ and hence both markings are distributionally equal.
	
	To show the converse, define the function $\wt{\mc M}':\,\NM^0 \longrightarrow [0, \infty)$ such that $\wt{\mc M}'(\varphi)$ denotes the second-smallest element in $\arg\max_{m' \ge 0}f(m',\varphi)$. If the latter set consists only of a single element, then $\wt{\mc M}'(\varphi)$ takes this value. This induces a marking $\wt\Psi = \{(X_i, M_i, \wt M_i')\}_{i}$ with $\wt M_i' = \wt{\mc M}'(\varphi)$, which is also intensity-optimal. Since we assumed optimal markings to be distributionally unique, we conclude that $\wt M_0' = M_0'$ holds $\P^0_\Phi$-almost surely. In other words, $\arg\max_{m' \ge 0}f(m',\Phi)$ is unique for $\P^0$-almost every realization of the base process $\Phi$. 
\end{proof}



%
%WR models
%
\subsection{Proofs of Propositions \ref{uniqThm} and \ref{nUniqThm}}
In this section, we prove Propositions \ref{uniqThm} and \ref{nUniqThm} on uniqueness and non-uniqueness in Widom-Rowlinson-type models. To establish Proposition~\ref{uniqThm}, we heavily rely on the one-dimensional problem setting, which allows us to construct effective shields against long-range interactions.

\begin{proof}[Proof of Proposition \ref{uniqThm}]
	The idea of proof is to construct shields against long-range dependence by considering blocks of adjacent sites that all have larger '$+$' than '$-$' marks. More precisely, a discrete interval $[i, j] \subset \Z$ is \emph{blocking} if
	\begin{enumerate}
		\item $M_k^+ > M_\ell^-$ for all $k, \ell \in [i, j]$, and
		\item $\sum_{i \le k \le j} M_k^+ > \sum_{i-1 \le k \le j+1} M_k^-$.
	\end{enumerate}
	Since the marks $\{M_k^+, M_k^-\}_{k \in \Z}$ are iid and absolutely continuous, blocking intervals occur with a positive intensity. Now, we assert that if $[i, j]$ is blocking, then there exists $k \in [i, j]$ such that $M_k' = +$ for every locally optimal thinning $\Psi$. Once this assertion is established, the proof of the theorem is complete. Indeed, if $k<\ell$ are such that $M_k' = M_\ell' = +$, then local optimality already dictates the  specific values of $M_m'$ for any $m \in [k, \ell]$.

	It remains to prove the assertion. For this purpose, we distinguish between different possible values of $M_{i-1}'$ and $M_{j+1}'$. If neither of them equals $-$, then we conclude from property (1) that $M_m' = +$ for all $m \in [i, j]$. Hence, we may assume for instance that $M_{i-1}' = -$. If additionally $M_{j+1}' = -$, then property (2) implies that there exists $m \in [i, j]$ with $M_m' = +$. We claim that for this choice of $m$, we still have $M_m' = +$, even if $M_{j+1} = +$ or $M_{j+1} = o$. Indeed, by property (1), there cannot exist $i \le i' \le j' \le j$ such that $M_{i'-1}' = M_{j'+1}' = o$ and $M_k' = -$ for all $k \in [i', j']$. Hence, there exists $m' \in [i, j]$ such that 
	$$M_k' = \begin{cases}
		- &\text{ if $i \le k < m'$},\\
		0 &\text{ if $ k = m'$},\\
		+ &\text{ if $m' < k \le j$}.\\
	\end{cases}$$
	In fact, now property (1) gives that $m' = i$, so that $M_m' = +$, as asserted.
\end{proof}

The conceptual reason behind the non-uniqueness of locally optimal markings lies in the non-amenability of $\B$. Loosely speaking, the boundary of a finite number of negative particles in an infinite sea of positive particles is so large that the fluctuation gains cannot compensate for the large losses incurred in the forbidden zone at the boundary.

\begin{proof}[Proof of Proposition \ref{nUniqThm}]
	For a vertex set $V \subset \B$ let $\partial V$ denote the vertex boundary of $V$, i.e., all vertices outside $V$ that are adjacent to a vertex in $V$. 
	We start from the marking $\Psi^+$ consisting entirely of pluses, i.e., $M_b' = +$ for all $b \in \B$. We claim that $\Psi^+$ is locally optimal. Since by symmetry, then the same is true for $\Psi^-$, establishing the claim will conclude the proof.

	Let $\Psi$ be an arbitrary marking disagreeing from $\Psi^+$ in finitely many points. That is, there exists a finite vertex set $V \subset \B$ such that in $\Psi$ we have
	\begin{enumerate}
		\item $M_b' = -$ for all $b \in V$,
		\item $M_b' = 0$ for all $b \in \partial V$, and
		\item $M_b' = +$ for all $b \in \B \setminus (V \cup \partial V)$. 
	\end{enumerate}
	Now, using induction argument, one can show that the non-amenability of the graph implies  that $\# \partial V \ge \# V$ for any $V \subset \B$. Since the marks are confined to the interval $[0.9, 1.1]$, we therefore conclude that 
	$$\Psi \Delta_{\B} \Psi^+ \le 1.1\#V - 0.9(\#V + \#\partial V) \le -0.7\#V < 0.$$
	Hence, $\Psi^+$ is locally optimal, as asserted.
\end{proof}
